Agent-FLAN: Designing Data and Methods of Effective Agent Tuning for Large Language Models

Open-sourced Large Language Models (LLMs) have achieved great success in various NLP tasks, however, they are still far inferior to API-based models when acting as agents. How to integrate agent ability into general LLMs becomes a crucial and urgent problem. This paper first delivers three key observations: (1) the current agent training corpus is entangled with both formats following and agent reasoning, which significantly shifts from the distribution of its pre-training data; (2) LLMs exhibit different learning speeds on the capabilities required by agent tasks; and (3) current approaches have side-effects when improving agent abilities by introducing hallucinations. Based on the above findings, we propose Agent-FLAN to effectively Fine-tune LANguage models for Agents. Through careful decomposition and redesign of the training corpus, Agent-FLAN enables Llama2-7B to outperform prior best works by 3.5\% across various agent evaluation datasets. With comprehensively constructed negative samples, Agent-FLAN greatly alleviates the hallucination issues based on our established evaluation benchmark. Besides, it consistently improves the agent capability of LLMs when scaling model sizes while slightly enhancing the general capability of LLMs. The code will be available at https://github.com/InternLM/Agent-FLAN.

==> figures/ablations-figure-2.tex <==
% argument #1: any options
\makeatletter
\newenvironment{customlegend}[1][]{%
    \begingroup
    % inits/clears the lists (which might be populated from previous
    % axes):
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}%
}{%
    % draws the legend:
    \pgfplots@createlegend
    \endgroup
}%

% makes \addlegendimage available (typically only available within an
% axis environment):
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

\begin{figure*}[t]
\pgfplotsset{width=4.3cm, height=6cm,
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
       \draw[##1,/tikz/.cd,yshift=-0.25em]
        (0cm,0cm) rectangle (7pt,0.8em);},
   },}
    \centering
    % \vspace{-10mm}
    \begin{tikzpicture}  
    \begin{groupplot}[
          group style={
          group name=plot,
          horizontal sep=6pt,
          vertical sep=0pt,
          group size=5 by 1},]
      \nextgroupplot[
            ybar,
            ymin=0, ymax=80,
            ytick={0, 20, 40, 60, 80},
            major x tick style = transparent,
            bar width=12pt,
            enlarge x limits=0.25,
            ylabel={Rel. Accuracy (\%)},
            symbolic x coords={Held-In},  
            xtick=data,  
            axis x line*=bottom,
            axis y line*=left,
            y label style={at={(axis description cs:-0.22,0.5)},anchor=south},
            % nodes near coords,  
            % nodes near coords align={vertical},  
            % nodes near coords style={font=\scriptsize},
            % legend cell align=left,
            %     legend style={
            %             % at={(5.7,1.05)},
            %             at={(1.7,1.05)},
            %             anchor=south,
            %             column sep=1ex,
            %             font=\small,
            %     }
            ]  
        \addplot[ybar, fill=beige,  postaction={}] coordinates {
            (Held-In, 6.9)
        };
        \addplot[ybar, fill=classicrose,  postaction={}] coordinates {
            (Held-In, 71.3)
        };  
        \addplot[ybar, fill=babyblue,  postaction={}] coordinates {
            (Held-In, 68.7)
        };  
        \addplot[ybar, fill=frenchblue,  postaction={}] coordinates {
            (Held-In, 73.1)
        };  
 
      \nextgroupplot[
            ybar,
            ymin=0, ymax=80,
            ytick={0, 10, 20, 30, 40, 50, 60, 70, 80},
            major x tick style = transparent,
            bar width=12pt,
            enlarge x limits=0.25,
            % ylabel={GSM8K solve rate (\%)},
            symbolic x coords={HotpotQA},  
            xtick=data,  
            axis x line*=bottom,
            axis y line*=left,
            y axis line style={opacity=0},
            ytick=\empty,
            % legend cell align=left,
            %     legend style={
            %             at={(0.0,1.05)},
            %             draw=none,
            %             anchor=south,
            %             column sep=1ex,
            %             font=\small,
            %     }
            ]  
        \addplot[ybar, fill=beige,  postaction={}] coordinates {
            (HotpotQA, 43.4)
        };
        \addplot[ybar, fill=classicrose,  postaction={}] coordinates {
            (HotpotQA, 42.8)
        };  
        \addplot[ybar, fill=babyblue,  postaction={}] coordinates {
            (HotpotQA, 48.8)
        };  
        \addplot[ybar, fill=frenchblue,  postaction={}] coordinates {
            (HotpotQA, 54.7)
        };  
        
      \nextgroupplot[
            ybar,
            ymin=0, ymax=80,
            ytick={0, 10, 20, 30, 40, 50, 60, 70, 80},
            major x tick style = transparent,
            bar width=12pt,
            enlarge x limits=0.25,
            % ylabel={GSM8K solve rate (\%)},
            symbolic x coords={SciWorld},  
            xtick=data,  
            axis x line*=bottom,
            axis y line*=left,
            y axis line style={opacity=0},
            ytick=\empty,
            % legend cell align=left,
                % legend style={
                %         at={(0.0,1.05)},
                %         draw=none,
                %         anchor=south,
                %         column sep=1ex,
                %         font=\small,
                % }
            ]  
        \addplot[ybar, fill=beige,  postaction={}] coordinates {
            (SciWorld, 16.2)
        };
        \addplot[ybar, fill=classicrose,  postaction={}] coordinates {
            (SciWorld, 37.6)
        };  
        \addplot[ybar, fill=babyblue,  postaction={}] coordinates {
            (SciWorld, 46.2)
        };  
        \addplot[ybar, fill=frenchblue,  postaction={}] coordinates {
            (SciWorld, 54.9)
        };  

      \nextgroupplot[
            ybar,
            ymin=0, ymax=80,
            ytick={0, 10, 20, 30, 40, 50, 60, 70, 80},
            major x tick style = transparent,
            bar width=12pt,
            enlarge x limits=0.25,
            % ylabel={GSM8K solve rate (\%)},
            symbolic x coords={WebArena},  
            xtick=data,  
            axis x line*=bottom,
            axis y line*=left,
            y axis line style={opacity=0},
            ytick=\empty,
            % nodes near coords,  
            % nodes near coords align={vertical},  
            % nodes near coords style={font=\scriptsize},
            % legend cell align=left,
                % legend style={
                %         at={(0.0,1.05)},
                %         draw=none,
                %         anchor=south,
                %         column sep=1ex,
                %         font=\small,
                % }
            ]  
        \addplot[ybar, fill=beige,  postaction={}] coordinates {
            (WebArena, 19.1)
        };
        % \addplot[ybar, fill=gray,  postaction={pattern=north east lines}] coordinates {
        %     (Few-shot evaluation, 46.3)
        % };  
        % \addplot[ybar, fill=gray,  postaction={}] coordinates {
        %     (Zero-shot evaluation, 43.8)
        % };  
        \addplot[ybar, fill=classicrose,  postaction={}] coordinates {
            (WebArena, 11.8)
        };  
        \addplot[ybar, fill=babyblue,  postaction={}] coordinates {
            (WebArena, 43.2)
        };  
        \addplot[ybar, fill=frenchblue,  postaction={}] coordinates {
            (WebArena, 74.5)
        };  

        ]
      \nextgroupplot[
            ybar,
            ymin=0, ymax=80,
            ytick={0, 10, 20, 30, 40, 50, 60, 70, 80},
            major x tick style = transparent,
            bar width=12pt,
            enlarge x limits=0.25,
            % ylabel={GSM8K solve rate (\%)},
            symbolic x coords={T-Eval},  
            xtick=data,  
            axis x line*=bottom,
            axis y line*=left,
            y axis line style={opacity=0},
            ytick=\empty,
            % nodes near coords,  
            % nodes near coords align={vertical},  
            % nodes near coords style={font=\scriptsize},
            % legend cell align=left,
                legend style={
                        at={(2.2,0.25)},
                        draw=none,
                        anchor=south,
                        column sep=1ex,
                        font=\small,
                }
            ]  
        \addplot[ybar, fill=beige,  postaction={}] coordinates {
            (T-Eval, 31.7)
        };
        \addplot[ybar, fill=classicrose,  postaction={}] coordinates {
            (T-Eval, 47.9)
        };  
        \addplot[ybar, fill=babyblue,  postaction={}] coordinates {
            (T-Eval, 71.5)
        };  
        \addplot[ybar, fill=frenchblue,  postaction={}] coordinates {
            (T-Eval, 76.4)
        };
        % \legend{
        %     Flan 2022 (ours),
        %     Flan 2021,
        %     T0++,
        %     Super-Natural Instructions,
        %     OPT-IML-Max 175B,
        %     }
        ]
        ]
    \end{groupplot}
    \node[below,color=forestgreen,font=\small] at (2.05,4.6) {\textbf{+1.8}};
    \node[below,color=forestgreen,font=\small] at (5.0,3.6) {\textbf{+6.0}};
    \node[below,color=forestgreen,font=\small] at (7.9,3.6) {\textbf{+8.8}};
    \node[below,color=forestgreen,font=\small] at (10.8,4.65) {\textbf{+31.4}};
    \node[below,color=forestgreen,font=\small] at (13.8,4.75) {\textbf{+4.0}};
    
    \begin{customlegend}[legend columns=-1,legend style={at={(13.2,-1.0)},draw=none,column sep=1ex},legend entries={Llama2-7B,AgentLM-7B,AgentTuning*,Agent-FLAN(Ours)}]
    \addlegendimage{black,fill=beige,ybar,ybar legend}
    \addlegendimage{black,fill=classicrose,ybar,ybar legend}
    \addlegendimage{black,fill=babyblue,ybar,ybar legend}
    \addlegendimage{black,fill=frenchblue,ybar,ybar legend}
    \addlegendimage{black,fill=gray!35,ybar,ybar legend}
    % \addlegendimage{red,fill=black!50!red,area legend}
    % \addlegendimage{red,fill=black!50!red,sharp plot}
    % \addlegendimage{red,fill=black!50!red,mark=*,sharp plot}
    % \addlegendimage{red,fill=black!50!red,ybar,ybar legend}
    \end{customlegend}
    
    \end{tikzpicture} 
    \caption{
    \textbf{Comparison of recent agent tuning approaches on Held-In, Held-Out tasks}. Performances are normalized with GPT-4 results for better visualization. * denotes our re-implementation for a fair comparison.}
    \label{fig:flan-vs-competitors}
\end{figure*}
